Learn How to Cook a New Recipe in a New House: Using Map Familiarization, Curriculum Learning, and Bandit Feedback to Learn Families of Text-Based Adventure Games

We consider the task of learning to play families of text-based computer adventure games, i.e., fully textual environments with a common theme (e.g. cooking) and goal (e.g. prepare a meal from a recipe) but with different specifics; new instances of such games are relatively straightforward for humans to master after a brief exposure to the genre but have been curiously difficult for computer agents to learn. We find that the deep Q-learning strategies that have been successfully leveraged for superhuman performance in single-instance action video games can be applied to learn families of text video games when adopting simple strategies that correlate with human-like learning behavior. Specifically, we build agents that learn to tackle simple scenarios before more complex ones using curriculum learning, that familiarize themselves in an unfamiliar environment by navigating before acting, and that explore uncertain environments more thoroughly using contextual multi-armed bandit decision policies. We demonstrate improved task completion rates over reasonable baselines when evaluating on never-before-seen games of that theme.

==> bertexamplefootnote.tex <==
\begin{figure*}[!th]
    \centering
    \footnotesize
    \begin{tabular}%
    {c>{\raggedright\arraybackslash}p{10cm}%
   >{\raggedleft\arraybackslash}p{4cm}%
  }
    &\textbf{Master} & \textbf{Player} \\ \hline
    &You find yourself in a kitchen. You make out a fridge. The fridge contains a yellow bell pepper. You see a cookbook and a knife on the table.  & examine cookbook \\
    &You open the cookbook and start reading. `Recipe 1: ingredients: red apple. directions: slice the red apple. prepare meal' & inventory \\
    \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textsc{BERT}}}}&You are carrying: a red apple, a red onion. & drop red onion. \\ \hline
    &you drop the red onion on the ground. & take knife from table.\\
    & you take the knife from the table. & slice red apple with knife.\\
    & you slice the red apple. your score has just gone up by one point. & prepare meal. \\
    & adding the meal to your inventory. your score has just gone up by one point. & eat meal.\\
    & you eat the meal. your score has just gone up by one point. you win. & \\ \hline
    \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textsc{base}}}}&You are carrying: a red apple, a red onion. & cook red apple with stove \\ 
    & You fried the red apple. You lost! \\
    \end{tabular}
    \caption{Comparison of BERT and baseline models on an example game from the dev set after 270,000 steps of training on tier 1 data; common steps are shown at the top.}
    \label{fig:bertexample}
\end{figure*}

==> bertexamplescript.tex <==
\begin{figure*}[!th]
    \centering
    \scriptsize
    \begin{tabular}%
    {c>{\raggedright\arraybackslash}p{10cm}%
   >{\raggedleft\arraybackslash}p{4cm}%
  }
    &\textbf{Master} & \textbf{Player} \\ \hline
    &You find yourself in a kitchen. You make out a fridge. The fridge contains a yellow bell pepper. You see a cookbook and a knife on the table.  & \\
    && examine cookbook \\
    &You open the cookbook and start reading. `Recipe 1: ingredients: red apple. directions: slice the red apple. prepare meal' & \\
    && inventory \\
    &You are carrying: a red apple, a red onion. & \\ \hline
     \parbox[t]{2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{\textsc{BERT}}}}&& drop red onion. \\
    &you drop the red onion on the ground. & \\
    && take knife from table. \\
    & you take the knife from the table. & \\
    && slice red apple with knife. \\
    & you slice the red apple. your score has just gone up by one point. & \\
    && prepare meal. \\
    & adding the meal to your inventory. your score has just gone up by one point. & \\
    && eat meal. \\
    & you eat the meal. your score has just gone up by one point. you win. & \\ \hline
    \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textsc{base}}}}&& cook red apple with stove \\
    & You fried the red apple. You lost! \\
    \end{tabular}
    \caption{Comparison of BERT and baseline models on an example game from the dev set after 270,000 steps of training on tier 1 data; common steps are shown at the top.}
    \label{fig:bertexample}
\end{figure*}

==> cooking-horiz.tex <==
\begin{figure*}[ht]
  \centering
  \begin{subfigure}[b]{0.33\linewidth}
    \centering\includegraphics[width=110pt]{learned-abilities-1.pdf}
    %\caption{\label{fig:fig1}}
  \end{subfigure}%
  \begin{subfigure}[b]{0.33\linewidth}
    \centering\includegraphics[width=110pt]{learned-abilities-2.pdf}
    %\caption{\label{fig:fig2}}
  \end{subfigure}%
   \begin{subfigure}[b]{0.33\linewidth}
    \centering\includegraphics[width=110pt]{learned-abilities-3.pdf}
    %\caption{\label{fig:fig2}}
  \end{subfigure}
   \begin{subfigure}[b]{0.33\linewidth}
    \centering\includegraphics[width=110pt]{learned-abilities-4.pdf}
    %\caption{\label{fig:fig2}}
  \end{subfigure}%
   \begin{subfigure}[b]{0.33\linewidth}
    \centering\includegraphics[width=110pt]{learned-abilities-5.pdf}
    %\caption{\label{fig:fig2}}
  \end{subfigure}%
   \begin{subfigure}[b]{0.33\linewidth}
    \centering\includegraphics[width=110pt]{learned-abilities-6.pdf}
    %\caption{\label{fig:fig2}}
  \end{subfigure}
  \caption{Comparison between BERT and baseline at learning six different cooking abilities. The BERT agent grasps most abilities much faster than the baseline.}
  \label{fig:bert-cnn-learn-abilities}
\end{figure*}


==> cooking-vert.tex <==
\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.5\linewidth}
    \centering\includegraphics[width=110pt]{learned-abilities-1.pdf}
    %\caption{\label{fig:fig1}}
  \end{subfigure}%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering\includegraphics[width=110pt]{learned-abilities-2.pdf}
    %\caption{\label{fig:fig2}}
  \end{subfigure}
   \begin{subfigure}[b]{0.5\linewidth}
    \centering\includegraphics[width=110pt]{learned-abilities-3.pdf}
    %\caption{\label{fig:fig2}}
  \end{subfigure}%
   \begin{subfigure}[b]{0.5\linewidth}
    \centering\includegraphics[width=110pt]{learned-abilities-4.pdf}
    %\caption{\label{fig:fig2}}
  \end{subfigure}
   \begin{subfigure}[b]{0.5\linewidth}
    \centering\includegraphics[width=110pt]{learned-abilities-5.pdf}
    %\caption{\label{fig:fig2}}
  \end{subfigure}%
   \begin{subfigure}[b]{0.5\linewidth}
    \centering\includegraphics[width=110pt]{learned-abilities-6.pdf}
    %\caption{\label{fig:fig2}}
  \end{subfigure}
  \caption{Comparison between BERT and baseline at learning six different cooking abilities. The BERT agent grasps most abilities much faster than the baseline.}
  \label{fig:bert-cnn-learn-abilities}
\end{figure}


==> curric-go-room-horiz.tex <==
\begin{figure*}[ht]
  \centering
  \begin{subfigure}[b]{0.35\linewidth}
    \centering\includegraphics[width=110pt]{tier1-dev.pdf}
    \caption{tier-1\label{fig:curr-tier-1}}
  \end{subfigure}%
  \begin{subfigure}[b]{0.35\linewidth}
    \centering\includegraphics[width=110pt]{tier2-dev.pdf}
    \caption{tier-2\label{fig:curr-tier-2}}
  \end{subfigure}%
   \begin{subfigure}[b]{0.35\linewidth}
    \centering\includegraphics[width=110pt]{tier3-dev.pdf}
    \caption{tier-3\label{fig:curr-tier-3}}
  \end{subfigure}
   \begin{subfigure}[b]{0.35\linewidth}
    \centering\includegraphics[width=110pt]{tier4-dev.pdf}
    \caption{tier-4\label{fig:curr-tier-4}}
  \end{subfigure}%
   \begin{subfigure}[b]{0.35\linewidth}
    \centering\includegraphics[width=110pt]{tier5-dev.pdf}
    \caption{tier-5\label{fig:curr-tier-5}}
  \end{subfigure}%
   \begin{subfigure}[b]{0.35\linewidth}
    \centering\includegraphics[width=110pt]{tier6-dev.pdf}
    \caption{tier-6\label{fig:curr-tier-6}}
  \end{subfigure}
  \caption{The training process of `curric go-room' broken down by tier. Results on tier-specific dev sets are shown. The learning is generally rational (scores and wins go up, steps go down) but is less effective in tiers 2 and 3.}
  \label{fig:curricgoroom}
\end{figure*}

==> curric-go-room-vert.tex <==
\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.5\linewidth}
    \centering\includegraphics[width=110pt]{tier1-dev.pdf}
    \caption{tier-1\label{fig:curr-tier-1}}
  \end{subfigure}%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering\includegraphics[width=110pt]{tier2-dev.pdf}
    \caption{tier-2\label{fig:curr-tier-2}}
  \end{subfigure}
   \begin{subfigure}[b]{0.5\linewidth}
    \centering\includegraphics[width=110pt]{tier3-dev.pdf}
    \caption{tier-3\label{fig:curr-tier-3}}
  \end{subfigure}%
   \begin{subfigure}[b]{0.5\linewidth}
    \centering\includegraphics[width=110pt]{tier4-dev.pdf}
    \caption{tier-4\label{fig:curr-tier-4}}
  \end{subfigure}
   \begin{subfigure}[b]{0.5\linewidth}
    \centering\includegraphics[width=110pt]{tier5-dev.pdf}
    \caption{tier-5\label{fig:curr-tier-5}}
  \end{subfigure}%
   \begin{subfigure}[b]{0.5\linewidth}
    \centering\includegraphics[width=110pt]{tier6-dev.pdf}
    \caption{tier-6\label{fig:curr-tier-6}}
  \end{subfigure}
  \caption{The training process of `curric go-room' broken down by tier. Results on tier-specific dev sets are shown. The learning is generally rational (scores and wins go up, steps go down) but is less effective in tiers 2 and 3.}
  \label{fig:curricgoroom}
\end{figure}
